One-parameter dynamical dark-energy from the generalized Chaplygin gas

The fact that Einstein's equations connect the space-time geometry to the total matter content of the cosmic substratum, but not to individual contributions of the matter species, can be translated into a degeneracy in the cosmological dark sector. Such degeneracy makes it impossible to distinguish cases where dark energy (DE) interacts with dark matter (DM) from a dynamical non-interacting scenario using observational data based only on time or distance measurements. In this paper, based on the non-adiabatic generalized Chaplygin gas (gCg) model, we derive and study some cosmological consequences of a varying one-parameter dynamical DE parameterization, which does not allow phantom crossing. We perform a parameter selection using the most recent public available data, such as the data from Planck 2018, eBOSS DR16, Pantheon and KiDS-1000. We find that current observations provide strong constraints on the model parameters, leading to values very close to the $\Lambda$CDM cosmology, at the same time that the well-known $\sigma_8$ tension is reduced from $\sim 3\sigma$ to $\sim 1\sigma$ level.

==> table_op1.tex <==
\begin{table*}[]
\renewcommand{\arraystretch}{1.3}
\centering
\begin{tabular}{c c c c c}
    \hline
    \hline
    \multicolumn{5}{c}{$\bar{w}$CDM} \\    
    %\hline
     & $\bar{w}_0$ & $\bar{\Omega}_m$ & $H_0$ & $S_8$ \\
    \hline
     SN Ia + BAO & $< -0.9924$ & $0.315 \pm 0.011$ & $70.5^{+1.4}_{-1.8}$  & - \\
     Weak Lensing & $< -0.902$ & $0.282^{+0.071}_{-0.090}$ & $72.9 \pm 5.0$ & $0.828^{+0.042}_{-0.073}$\\
     CMB & $< -0.99745$ & $0.3199^{+0.0080}_{-0.0099}$ & $66.90^{+0.72}_{-0.60}$ & $0.833 \pm 0.013$\\
    \hline
    \multicolumn{5}{c}{$w$CDM} \\
    %\hline
     & $\bar{w}_0$ & $\bar{\Omega}_m$ & $H_0$ & $S_8$ \\
    \hline
     SN Ia + BAO & $-1.01_{-0.009}^{+0.008}$ & $0.258_{-0.0157}^{+0.014}$ & $68.5_{}^{}$  & - \\
     Weak Lensing &  &  &  & \\
     CMB &  &  &  & \\
    \hline
    \hline
\end{tabular}
\caption{Best fit and $1\sigma$ confidence level for each sample used. }
\label{tab.results}
\end{table*}

==> table_op2.tex <==
\begin{table*}[]
\renewcommand{\arraystretch}{1.3}
\centering
\begin{tabular}{c c c c c | c c c c}
    \hline
    \hline
    & \multicolumn{4}{c}{$\bar{w}CDM$} & \multicolumn{4}{c}{$w$CDM}\\
    \hline
    & $\bar{w}_0$ & $\bar{\Omega}_m$ & $H_{0}$ & $S_{8}$ & $w_{0}$ & $\Omega_{m}$ & $H_{0}$ & $S_{8}$ \\
    SNIa $+$ BAO & $< -0.9924$ & $0.315 \pm 0.011$ & $70.5^{+1.4}_{-1.8}$ & - & $-1.01_{-0.009}^{+0.008}$ & $0.258_{-0.0157}^{+0.014}$ & $68.5_{}^{}$ & - \\
    Weak Lensing & $< -0.902$ & $0.282^{+0.071}_{-0.090}$ & $72.9 \pm 5.0$ & $0.828^{+0.042}_{-0.073}$ & & & & \\
    CMB & & & & & & & & \\
    \hline
    \hline
\end{tabular}
\caption{Best fit and $1\sigma$ confidence level for each sample used. }
\label{tab.results}
\end{table*}
